Detecting Cosmic Strings with Lensed Fast Radio Bursts

Correlated red noise recently reported from pulsar timing observations may be an indication of stochastic gravitational waves emitted by cosmic strings that formed during a primordial phase transition near the Grand Unification energy scale. Unfortunately, known probes of cosmic strings, namely the Cosmic Microwave Background anisotropies and string lensing of extragalactic galaxies, are not sensitive enough for low string tensions of $G\mu = 10^{-10}-10^{-7}$ that are needed to explain this putative signal. We show that strong gravitational lensing of Fast Radio Bursts (FRBs) by cosmic strings is a potentially unambiguous avenue to probe that range of string tension values. The image pair of string lensing are expected to have identical magnification factor and parity, and have a typical time delay of $\sim 10^2\,\,(G\,\mu/10^{-8})^2$ seconds. The unique spectral fingerprint of each FRB, as well as the possibility to detect correlations in the time series of the electric field of the radio waves, will enable verification of the string lensing interpretation. Very-Long-Baseline Interferometry (VLBI) observations can spatially resolve the image pair and provide a lower bound on the string tension based on the image separation. We calculate the FRB lensing rate as a function of FRB detection number for several different models of the FRB redshift distribution. We find that a survey detecting $\sim 10^5$ FRBs, in line with estimates for the detection rate of the forthcoming survey CHORD, can uncover a strong lensing event for a string tension of $G\mu \simeq 10^{-7}$. Larger FRB surveys, such as Phase 2 of the Square Kilometre Array (SKA), have the potential to significantly improve the sensitivity on the string tension to $G\mu \simeq 10^{-9}$.

==> Efieldcorr.tex <==

On the other hand, one can correlate the electric field between the two bursts to confirm they are lensed. The decoherence will be discussed in the following to understand the condition of maintaining coherence.

First, if the lens resolves the FRB or emitting region $\ell_{FRB}$, the correlations are more complicated as the ordering of the different resolved geometric paths from the emitting region will be different for the two images. %{\bf [Think about whether this delay effect can be deconvolved/detected in correlation function of intensity]}
The condition to be unresolved means that
\begin{equation}
    \ell_{FRB} \lesssim \frac{\lambda}{\theta_E d_{L}} d_{LS} \sim 10^9 {\rm cm} \left( \frac{\lambda}{20 cm} \right)  \left(\frac{G\mu}{10^{-8}}\right)^{-1}.
\end{equation}
%where the last evaluation we have have dropped order unity factors that arise from there being different distances.  
This condition is satisfied for much larger emitting regions than the $\sim 10$km size of a neutron star, which is the expected distance in magnetospheric models for FRB emission.  The other class of FRB emission models where the FRB originates from a shock external to the magnetar.  Taking the most developed synchrotron blast model \cite{Metzger:2019una}, the emission region may be at $R_{em} = 10^{12}-10^{13}$ cm from the FRB and come from Lorentz factors of $\Gamma =10^{2}-10^3$, such that  $\ell_{FRB} = R_{em}/\Gamma = 10^9-10^{11}$, which is resolved for $G\mu =10^{-8}$ but not smaller.\footnote{External shock models have trouble explaining the FRBs that have durations of microseconds \citep{} as the duration should be greater than $\ell_{FRB}/c/\Gamma$.}   

Scattering in the FRB host galaxy can make the effective size of the FRB image (`emitting region') larger with this size related to the scattering timescale by $c t_{sc} \sim \theta_{screen}^2 d_{screen}$ where $\theta_{screen}$ is the angle from the FRB to the illuminated part of the scattering screen at a distance $d_{screen}$.  Then the effective size of the FRB emisison region becomes $\ell_{FRB} =  \theta_{screen} d_{screen} = \sqrt{c t_{sc} d_{screen}} $.  Taking 1 ms scattering timescale, characteristic of tens of percent of bursts (but many are much smaller) and putting the screen at 1 pc results in $\ell_{FRB} = 10^{13} (d_{screen}/1pc)^{1/2}$~cm.  Tenth's of parsec is roughly the size of the magnetar nebulae on your timsescales (or a dense HII region).  (This scattering timescale is large so that it likely is not the ISM at 10s of parsecs.)  Thus, for $G\mu = 10^{-8}$ the host scattering needs to occur on A.U. scales or some bursts need to be unscattered.   This difficulty may only apply to some FRBs as there is no evidence for scattering for many FRBs, with limits of $t_{sc}\lesssim 1\mu s$ for some.  Futuristic surveys sensitive to $G\mu = 10^{-11}$, millisecond scattering delays from a screen as far as a parsec from the host will be unresolved.

Scattering from multipath propogation in the Milky Way can also wash out phase correlations between the two string-lensed images. A characteristic scattering timescale out of the disk of the Galaxy is $\sim 10^{-7}  \nu_{\rm GHz}^{-4}$seconds.  Thus, by $10$GHz, scattering is not relevant as this becomes smaller than the period of a wave, $\nu^{-1}$, and so all paths correlate.  It is much harder to survey the sky at $10$GHz than $\lesssim 1$GHz as the instrumental beam of a radio telescope is much smaller, so here we consider whether correlations are expected even when the scattering timescale is large.    


So, let us consider the effect of scattering as the FRB light travels through the Milky Way.  Then, phases are acquired from inhomogeneities in the density can lead to decoherence of the electric field.  The Fresnel scale is the distance over which the phase of the geometric path differs by $2\pi$ or $R_F = \sqrt{\lambda d_{MW}/2\pi}$, where for $d_{MW} \sim 100 pc$ then $R_F \sim 10^{10.5} \nu_{GHz}^{-1/2}$cm. In the limit of strong scattering such that inhomogeneities in the denisty lead to larger than $2\pi$ phase accumulations on separations smaller than $R_F$ the size of the FRB light comes from a region of size $R_{ref} = R_F^2/R_{\rm diff}$ where $R_{\rm diff}$ is the scale at which phase variations are greater than $2\pi$ that is related to the density inhomgeneties.  To get the observed microsecond scattering in the MW, $R_{\rm diff} \sim 10^{11} \nu_{GHz}^{-2}cm $ such that $R_{ref} = 10^{11.5} \nu_{GHz}$cm. In the limit of many images from strong scattering, the correlation of the electric field between the two (unresolved by lens) bursts $\langle E_1^* E_2 \rangle$ is going to be the fraction of images that they share.   Thus, it will go like $(R_{ref}/[\theta_E d_{MW}])^2 \sim 0.01 [G \mu]_{-8}^{-1}\nu_{GHz}^2$.  If the noise is set by the FRB (that it dominates over backgorund noise temperature), which probably holds for an FRB and sensitive instrument, correlations as large as one over the square root of the number of samples $N_{sample} = \sqrt{\nu \tau_{FRB}}$ can be detected or $\sim 10^{-3}$ for a milisecond burst at a GHz.
%{\bf [This assumes all the information is in the zero lag correlation function and the properties of all the images are essentially the same despite coming from two directions.  I suspect both are true but don't know. ]}

The conclusion is that coherence is likely to maintain at a GHz, and very likely at a few GHz.  The biggest complication may be the distance to the scattering screen in the host, but should not change the conclusion.
